ReverseMath: Answer Inversion for Scalable and Verifiable Mathematical Problem Generation

Mathematical reasoning benchmarks are vital for evaluating large language models (LLMs), but many are static and repeatedly exposed through public evaluation and training pipelines, making it difficult to separate genuine reasoning from memorization. Meanwhile, manually constructing new math problems with reliable answers remains costly. We introduce ReverseMath, a scalable method for generating new math problems through answer inversion. Given a problem and its answer, ReverseMath masks a numerical value in the original problem, treats the original answer as a known condition, and rewrites the problem so that the masked value becomes the new answer. The generated problem reverses the original input-output relation, making its answer known by construction. We study ReverseMath for both evaluation and training. For evaluation, paired original/reversed problems reveal substantial behavioral shifts: models sometimes fail on reversed problems and even incorrectly output the original answer, suggesting memorization-like behavior. For training, ReverseMath provides automatically labeled reversed problems as data augmentation for reinforcement learning (RL). Experiments show that including ReverseMath-generated data improves mathematical reasoning performance across multiple benchmarks, demonstrating its value as both an analysis tool and a scalable source of verifiable training data.

==> old_intro.tex <==
\section{Introduction}

Recent advances in large language models (LLMs) have led to substantial improvements in mathematical reasoning tasks \cite{llm_math1,llm_math2}. Despite these gains, it remains unclear whether strong benchmark performance reflects genuine reasoning ability or reliance on memorization of problem patterns \cite{memorization1,memorization2}. As models continue to scale, this ambiguity poses a growing challenge for reliable evaluation.

A key limitation of current evaluation practices is that widely used benchmarks are largely static. Since these datasets are publicly available and reused extensively, models are increasingly likely to encounter similar problem instances during training \cite{data_contamination1}. As a result, high performance may be partially driven by memorization rather than true generalization \cite{data_contamination2}. Moreover, constructing new mathematical reasoning problems typically requires substantial human effort, making it difficult to maintain up-to-date and diverse evaluation data.

To address these challenges, we seek a practical and scalable approach for generating new mathematical reasoning problems from existing benchmarks. Ideally, such a method should (1) produce diverse and challenging problem instances, (2) provide reliable ground-truth answers without manual annotation, and (3) enable systematic analysis of model behavior beyond aggregate accuracy.

In this work, we propose a simple yet effective \textit{answer-conditioned problem generation} framework. Our key idea is to transform a solved problem into a new one by converting its answer into a known fact and redefining the target of inference. Concretely, given an original problem, we mask a numerical variable and provide the original answer as context. We then prompt a language model to generate a new problem in which the original answer becomes part of the given information, and the goal is to recover the masked variable.

This transformation produces a new problem instance with a different answer and a modified reasoning process. Importantly, the generated problem is not a paraphrase of the original, but a new instance that requires different reasoning steps while remaining semantically related. Furthermore, since the target variable is known by construction, the answer to the generated problem is deterministic, eliminating the need for manual annotation.

The resulting data provides multiple benefits. First, the transformation often induces reverse or inverse reasoning, enabling the construction of systematically more challenging problems. Second, by maintaining the relationship between original and generated instances, our framework naturally produces structured problem pairs that support the analysis of memorization. Differences in model performance across such pairs can reveal reliance on surface patterns rather than robust reasoning. Finally, the generated data can be used as an effective resource for training augmentation, improving model performance on mathematical reasoning tasks \cite{data_augmentation1}.

Empirically, we observe that model predictions often differ substantially between original and generated problems, even when they are semantically related. This highlights limitations that are not captured by standard evaluation metrics and underscores the importance of scalable data generation for reliable evaluation. Overall, our framework converts existing benchmarks into a renewable source of diverse, verifiable, and structurally varied reasoning problems.

\paragraph{Contributions.}
Our contributions are as follows:

% method
% as evaluation
% as training augmentation
\begin{itemize}
    \item We propose a fully automated answer-conditioned framework for generating new mathematical reasoning problems from existing benchmarks.
    \item We introduce a transformation that converts solved problems into new instances with different targets and reasoning processes, while providing deterministic answers.
    \item We show that the generated data enables both harder problem construction and systematic analysis of memorization through structured comparisons.
    \item We demonstrate that the generated data can be used for training augmentation, improving mathematical reasoning performance.
\end{itemize}
